Hyperpolarization read-out through rapidly rotating fields in the zero- and low-field regime

An integral part of para-hydrogen induced polarization (PHIP) methods is the conversion of nuclear singlet order into observable magnetization. In this study polarisation transfer to a heteronucleus is achieved through a selective rotation of the proton singlet-triplet states driven by a combination of a rotating magnetic field and a weak bias field. Surprisingly we find that efficient polarisation transfer driven by a STORM (Singlet-Triplet Oscillations through Rotating Magnetic fields) pulse in the presence of $\mu$T bias fields requires rotation frequencies on the order of several kHz. The rotation frequencies therefore greatly exceed any of the internal frequencies of typical zero- to ultralow field experiments. We further show that the rotational direction of the rotating field is not arbitrary and greatly influences the final transfer efficiency. Some of these aspects are demonstrated experimentally by considering hyperpolarised (1-$^{13}$C)fumarate. In addition, we provide numerical simulations highlighting the resilience of the STORM pulse against disruptive quadrupolar coupling partners. In contrast to most of the existing methods, the STORM procedure therefore represents a promising candidate for quadrupolar decoupled polarisation transfer in PHIP experiments.

==> Figures/decoupling.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{Graphics/Decoupling_v2.pdf}
\caption{\label{fig:decoupling} Numerically simulated polarization build-up curves for a system containing two protons in the singlet state coupled to a \Cth nucleus. The spin-spin couplings agree with those of (1-\Cth)fumarate. In addition one of the protons is coupled to a deuteron spin with a $J$-coupling constant of 2.5~Hz. Individual pulse sequence parameters for the simulations have been optimised for (1-\Cth)fumarate ignoring the additional deuteron spin.}
\end{figure}
